Image-Driven Biophysical Tumor Growth Model Calibration

We present a novel formulation for the calibration of a biophysical tumor growth model from a single-time snapshot, MRI scan of a glioblastoma patient. Tumor growth models are typically nonlinear parabolic partial differential equations (PDEs). Thus, we have to generate a second snapshot to be able to extract significant information from a single patient snapshot. We create this two-snapshot scenario as follows. We use an atlas (an average of several scans of healthy individuals) as a substitute for an earlier, pretumor, MRI scan of the patient. Then, using the patient scan and the atlas, we combine image-registration algorithms and parameter estimation algorithms to achieve a better estimate of the healthy patient scan and the tumor growth parameters that are consistent with the data. Our scheme is based on our recent work (Scheufele et al, "Biophysically constrained diffeomorphic image registration, Tumor growth, Atlas registration, Adjoint-based methods, Parallel algorithms", CMAME, 2018), but apply a different and novel scheme where the tumor growth simulation in contrast to the previous work is executed in the patient brain domain and not in the atlas domain yielding more meaningful patient-specific results. As a basis, we use a PDE-constrained optimization framework. We derive a modified Picard-iteration-type solution strategy in which we alternate between registration and tumor parameter estimation in a new way. In addition, we consider an $\ell_1$ sparsity constraint on the initial condition for the tumor and integrate it with the new joint inversion scheme. We solve the subproblems with a reduced-space, inexact Gauss-Newton-Krylov/quasi-Newton methods. We present results using real brain data with synthetic tumor data that show that the new scheme reconstructs the tumor parameters in a more accurate and reliable way compared to our earlier scheme.

==> makefile <==
filename=SIAM-SISC_moving_atlas
compPdftex=pdflatex

all: 
	${compPdftex} ${filename}

bib:
	pdflatex ${filename}
	bibtex ${filename}
	${compPdftex} ${filename}
	${compPdftex} ${filename}
	@echo Done ....!

clean:
	rm -f *.aux *.log *.dvi *.blg *.bbl \
          *.fls *.fdb_latexmk *.out *.spl    \
          *.brf *.snm *.toc *.nav       \
		  *.pdfsync *.pdf 
	@echo Cleaned ....! 

%.pdf: %.tex
	${compile} $*
	${compile} $* 


